Adaptive Distributed Filtering of DDoS Traffic on the Internet

Despite the proliferation of traffic filtering capabilities throughout the Internet, attackers continue to launch distributed denial-of-service (DDoS) attacks to successfully overwhelm the victims with DDoS traffic. In this paper, we introduce a distributed filtering system that leverages nodes distributed along the paths of DDoS traffic to filter the DDoS traffic. In particular, we focus on adaptive distributed filtering, a new direction in filtering DDoS traffic. In our design, a subscriber to the distributed filtering service can act on behalf of a DDoS victim and generate filtering rules that not only adapt to the most suitable and effective filtering granularity (e.g., IP source address and a port number vs. an individual IP address vs. IP prefixes at different lengths), but also adapt to the preferences of the subscriber (e.g., maximum coverage of DDoS traffic vs. minimum collateral damage from dropping legitimate traffic vs. minimum number of rules). We design an efficient algorithm that can generate rules adaptive toward filtering granularities and objectives, which can further help determine where to deploy generated rules for the best efficacy. We evaluated our system through both large-scale simulations based on real-world DDoS attack traces and pilot studies. Our evaluations confirm that our algorithm can generate rules that adapt to every distinct filtering objective and achieve optimal results. We studied the success rate and distribution of rule deployment under different Internet-scale rule deployment profiles, and found a small number of autonomous systems can contribute disproportionately to the defense. Our pilot studies also show our adaptive distributed filtering system can effectively defend against real-world DDoS attack traces in real time.

==> Makefile <==
export TEXINPUTS=.//:
#export BSTINPUTS=.//:
PDFLATEXSW = -shell-escape

BASE    =       main
#BASE    =       drawbridge

all:
	pdflatex $(PDFLATEXSW) $(BASE)
	-bibtex $(BASE)
	pdflatex $(PDFLATEXSW) $(BASE)
	pdflatex $(PDFLATEXSW) $(BASE)

once:
	pdflatex $(PDFLATEXSW) $(BASE)

env:
	@echo ${BSTINPUTS}

clean:
	$(RM) -f *.ilg *.log *.dvi *.bbl *.aux *.blg *.X??? *.out *.ps *.gz *.fls *.fdb_latexmk $(BASE).pdf 
	find . -name \*eps-converted-to.pdf -type f -delete

